Finite-coupling spectrum of O(N) model in AdS

We determine the scaling dimensions in the boundary $\mathsf{CFT}_{d}$ corresponding to the $\mathsf{O}(N)$ model in $\mathsf{EAdS}_{d+1}$. The $\mathsf{CFT}$ data accessible to the 4-point boundary correlator of fundamental fields are extracted in $d=2$ and $d=4$, at a finite coupling, and to the leading nontrivial order in the $1/N$ expansion. We focus on the non-singlet sectors, namely the anti-symmetric and symmetric traceless irreducible representations of the $\mathsf{O}(N)$ group, extending the previous results that considered only the singlet sector. Studying the non-singlet sector requires an understanding of the crossed-channel diagram contributions to the $s$-channel conformal block decomposition. Building upon an existing computation, we present general formulas in $d=2$ and $d=4$ for the contribution of a $t$-channel conformal block to the anomalous dimensions of $s$-channel double-twist operators, derived for external scalar operators with equal scaling dimensions. Up to some technical details, this eventually leads to the complete picture of $1/N$ corrections to the $\mathsf{CFT}$ data in the interacting theory.

==> preamble/tikz-diagrams.tex <==
\usepackage{tikz}
\usetikzlibrary{positioning,calc}
\usetikzlibrary{arrows,arrows.meta}
\usetikzlibrary{decorations.pathmorphing,decorations.markings}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{patterns, patterns.meta}
\usetikzlibrary{fadings}

%% Tiny space in math mode
\NewCommandCopy{\WD@dotaccent}{\.}
\ProvideDocumentCommand{\.}{}{\TextOrMath{\WD@dotaccent}{\mspace{1mu}}}

\RequirePackage[outline]{contour} % for text outlines
\contourlength{0.08em}

%% Define common styles
%% Inspired by Julien Barrat's PhD thesis https://inspirehep.net/literature/2749545
\definecolor{OPEcolor}{RGB}{220,249,250}
\def\WD@dlWidth{1.2pt} % default width for exchange double lines
\tikzset{
    label distance=0.8ex,
    every label/.style = {anchor=mid},
    thinline/.style  = {line width=0.85pt, draw=black, line cap=round},
    line/.style      = {line width=1pt,   draw=black},
    thickline/.style = {line width=1.5pt, draw=black},
    overline/.style  = {line width=1.5pt, double distance=1pt, draw=white, double=black},
    dashline/.style  = {line width=1pt,   draw=black, densely dashed},
    dotline/.style   = {line width=1pt,   draw=black, loosely dotted},
    doubleline/.style= {line width=0.8pt, double distance between line centers=1.4*\WD@dlWidth, double},
    doublefilled/.style = {
        pattern={Lines[angle=#1+45,distance=1.4pt,line width=0.4pt]},
        pattern color=darkgray, line width=0.8pt, draw=black
    },
    wave/.style = {line width=1pt, draw=black, decorate, decoration={snake, amplitude=1.5pt, segment length=5pt, pre length=#1}},
    correlator/.style    = {
        draw, circle, line width=0.8pt,
        % pattern={Lines[angle=45,distance=2.5pt,line width=0.5pt]},
        % pattern=crosshatch, pattern color=black!60,
        inner color=black!30, outer color=black!5,
    },
    boundarypoint/.style = {draw, circle, fill=white,     line width=0.6pt, scale=.4},
    bulkpoint/.style     = {draw, circle, fill=black!80,  line width=0.6pt, scale=.35},
    % bulkpoint/.style     = {draw, circle, fill=white,     line width=0.8pt, scale=.36, minimum size=10pt, path picture={\fill[black!90] (0,0) circle[radius=2.5pt];}},
    vertex/.style        = {draw, circle, fill=lightgray, line width=0.8pt, scale=.5},
    vertexphi/.style     = {draw, circle, fill=black!60,  line width=0.8pt, scale=.35},
    vertexsubtle/.style  = {circle, fill=black!80, fill opacity=0.20, scale=.65},
    opevertex/.style     = {draw, circle, fill=OPEcolor,  line width=0.6pt, scale=.4},
    hide labels/.style = {every label/.append style={text opacity=0, xscale=0.5}},
}
\tikzset{ % custom dotted line with round dots - https://tex.stackexchange.com/a/101263
    dots/.style = {
        line width=1pt,
        line cap=round,
        dash pattern=on 0pt off #1,
    },
    dots/.default={4pt},
}


%%% Witten Diagrams

\NewExpandableDocumentCommand{\WD@smallerfactor}{}{0.9}
\newif\ifsmallerWD
\smallerWDfalse

%% Radius of the Witten Diagram circle (also used for Partial Waves)
\NewExpandableDocumentCommand{\WD@rDefault}{}{0.65cm}
%% Paddings around the Witten Diagram circle
\NewExpandableDocumentCommand{\WD@xpadNoIndices}{}{0.4ex}
\NewExpandableDocumentCommand{\WD@ypadNoIndices}{}{0.4ex}
\NewExpandableDocumentCommand{\WD@xpadWithIndices}{}{0.5em}
\NewExpandableDocumentCommand{\WD@ypadWithIndices}{}{0.6ex}
%% Helper macro to set the scaling factor for Witten Diagrams
\NewDocumentCommand{\WD@SetupScaling}{m m}{% #1: starred, #2: scaling factor
    \ifsmallerWD\def\WD@r{#2*\WD@smallerfactor*\WD@rDefault}
    \else       \def\WD@r{#2*\WD@rDefault}\fi
    \def\WD@xpad{#2*\WD@xpadNoIndices}
    \def\WD@ypad{#2*\WD@ypadNoIndices}
    \IfBooleanT{#1}{ % if we have indices, use larger padding
        \def\WD@xpad{#2*\WD@xpadWithIndices}
        \def\WD@ypad{#2*\WD@ypadWithIndices}
    }
}

%% enlarge bounding box by given padding
\NewDocumentCommand{\WD@ExpandBoundingBox}{O{\WD@xpad}O{\WD@ypad}}{
    \useasboundingbox ([shift={(-#1,-#2)}]current bounding box.south west)
    rectangle         ([shift={( #1, #2)}]current bounding box.north east);
}

%% boundary points/nodes of the Witten Diagram circle
\NewDocumentCommand{\WD@BoundaryPoints}{m}{% #1: starred (omit labels)
    \begin{scope}[overlay, \IfBooleanF{#1}{hide labels}]
        \node[boundarypoint,label={145:$    i\.  $}] at (145:\WD@r) (e1) {};
        \node[boundarypoint,label={215:$    j\.\.$}] at (215:\WD@r) (e2) {};
        \node[boundarypoint,label={ 35:$\.\.k    $}] at ( 35:\WD@r) (e3) {};
        \node[boundarypoint,label={325:$  \.l    $}] at (325:\WD@r) (e4) {};
    \end{scope}
}

%% 4-point correlator (stared version shows boundary labels, optional argument for central label)
\tikzfading[name=radial fade 70, inner color=transparent!70, outer color=transparent!100]
\NewDocumentCommand{\FourPt}{s O{} O{1}}{%
    \WD@SetupScaling{#1}{#3}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \draw[line] (0,0) circle [radius=\WD@r];
        \WD@BoundaryPoints{#1}
        \draw[line] (e2) -- (e3);
        \draw[line] (e1) -- (e4);
        \draw[correlator] (0,0) circle [radius=5/8*\WD@r];
        \fill[fill=black!20, path fading=radial fade 70] (0,0) circle [radius=1/3*\WD@r];
        \IfBlankF{#2}{\node at (0,0) {\contour*{black!10}{#2}};}
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}
\NewDocumentCommand{\tExchContrib}{s O{} O{1}}{%
    \WD@SetupScaling{#1}{#3}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \draw[line] (0,0) circle [radius=\WD@r];
        \coordinate (B) at (0,-3/8*\WD@r);
        \coordinate (T) at (0, 3/8*\WD@r);
        \WD@BoundaryPoints{#1}
        \draw[line] (e2) -- (B);
        \draw[line] (e1) -- (T);
        \draw[line] (e3) -- (T);
        \draw[line] (e4) -- (B);
        \draw[correlator] (0,0) circle [x radius=1/3*\WD@r, y radius=5/8*\WD@r];
        \fill[fill=black!20, path fading=radial fade 70] (0,0) circle [x radius=1/5*\WD@r, y radius=1/3*\WD@r];
        \IfBlankF{#2}{\node at (0,0) {\contour*{black!10}{#2}};}
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}

%% Disconected Contributions (starred version shows boundary labels)
\NewDocumentCommand{\sDisc}{s O{1}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \draw[line] (0,0) circle [radius=\WD@r];
        \WD@BoundaryPoints{#1}
        \draw[line] (e2) to[out=  60,in=-60] (e1);
        \draw[line] (e3) to[out=-120,in=120] (e4);
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}
\NewDocumentCommand{\tDisc}{s O{1}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \draw[line] (0,0) circle [radius=\WD@r];
        \WD@BoundaryPoints{#1}
        \draw[line] (e2) to[out= 25,in= 155] (e4);
        \draw[line] (e1) to[out=-25,in=-155] (e3);
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}
\NewDocumentCommand{\uDisc}{s O{1}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \draw[line] (0,0) circle [radius=\WD@r];
        \WD@BoundaryPoints{#1}
        \draw[line]     (e2) -- (e3);
        \draw[overline] (e1) -- (e4);
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}

%% helper macro to create 4 corner nodes for vertex diagrams
\NewDocumentCommand{\cornernodes}{O{0.8}}{
    \begin{scope}[overlay]
        \node[scale=0.4] at (135:#1*\WD@r) (e1) {};
        \node[scale=0.4] at (225:#1*\WD@r) (e2) {};
        \node[scale=0.4] at ( 45:#1*\WD@r) (e3) {};
        \node[scale=0.4] at (315:#1*\WD@r) (e4) {};
    \end{scope}
}
%% (phi^2)^2 vertex
\NewDocumentCommand{\vertexPhi}{s O{1}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \node[vertexphi] at (0,0) (V) {};
        \cornernodes
        \draw[line] (e1) -- (V);
        \draw[line] (e2) -- (V);
        \draw[line] (e3) -- (V);
        \draw[line] (e4) -- (V);
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}
\NewDocumentCommand{\vertexPhiChannelS}{s O{1}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \cornernodes
        \draw[line, rounded corners=3pt] (e1) -- (0,0) -- (e2);
        \draw[line, rounded corners=3pt] (e3) -- (0,0) -- (e4);
        \node[vertexsubtle] at (0,0) (V) {};
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}
\NewDocumentCommand{\vertexPhiChannelT}{s O{1}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \cornernodes
        \draw[line, rounded corners=3pt] (e1) -- (0,0) -- (e3);
        \draw[line, rounded corners=3pt] (e2) -- (0,0) -- (e4);
        \node[vertexsubtle] at (0,0) (V) {};
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}
\NewDocumentCommand{\vertexPhiChannelU}{s O{1}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \cornernodes
        \draw[line]     (e2) -- (e3);
        \draw[overline] (e1) -- (e4);
        \node[vertexsubtle] at (0,0) (V) {};
        \WD@ExpandBoundingBox[0.7*\WD@xpad][0.5*\WD@ypad] % slightly enlarge bounding box
    }
}

\NewDocumentCommand{\phiLoop}{s O{1}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \def\WD@rloop{0.45*\WD@r} % radius of the loop
        \node at (0,0) (O) {$\scriptstyle\color{gray}n\.$};
        \draw[line] (0,0) circle [radius=\WD@rloop];
        \draw[doubleline]             (\WD@rloop,0) -- (0.9*\WD@r,0);
        \draw[doubleline, rotate= 80] (\WD@rloop,0) -- (0.9*\WD@r,0);
        \draw[doubleline, rotate=-80] (\WD@rloop,0) -- (0.9*\WD@r,0);
        % \draw[doublefilled]                 (\WD@rloop,-\WD@dlWidth) rectangle (0.9*\WD@r,+\WD@dlWidth);
        % \draw[doublefilled=-10, rotate= 80] (\WD@rloop,-\WD@dlWidth) rectangle (0.9*\WD@r,+\WD@dlWidth);
        % \draw[doublefilled= 10, rotate=-80] (\WD@rloop,-\WD@dlWidth) rectangle (0.9*\WD@r,+\WD@dlWidth);
        \node[vertex] at (  0:\WD@rloop) (v1) {};
        \node[vertex] at ( 80:\WD@rloop) (v2) {};
        \node[vertex] at (-80:\WD@rloop) (v3) {};
        \node at (  0:1.2*\WD@r) (l1) {$\sigma$};
        \node at ( 80:1.2*\WD@r) (l2) {$\sigma$};
        \node at (-80:1.2*\WD@r) (l3) {$\sigma$};
        % fill rest with dots
        \draw[line width=1.5pt,white] ([shift=(120:\WD@rloop)]0,0) arc [radius=\WD@rloop, start angle=120, end angle=240];
        \draw[dashline] ([shift=(135:\WD@rloop)]0,0) arc [radius=\WD@rloop, start angle=135, end angle=250];
        \draw[dots=4.24pt, gray] ([shift=(105:0.7*\WD@r)]0,0) arc [radius=0.7*\WD@r, start angle=105, end angle=260];
        % \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}

%% free sigma propagator
\NewDocumentCommand{\SigmaFreePropag}{s O{1.2}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \coordinate (L) at (-3/8*\WD@r,0);
        \coordinate (R) at ( 3/8*\WD@r,0);
        \draw[doubleline] (L) -- (R);
        \node[boundarypoint] at (L) (e1) {};
        \node[boundarypoint] at (R) (e2) {};
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}
%% bubble between two free sigma propagators
\NewDocumentCommand{\SigmaFreeBubble}{s O{1.0}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \node[boundarypoint] at (-10/8*\WD@r,0) (LL) {};
        \node[vertex]        at ( -4/8*\WD@r,0)  (L) {};
        \node[vertex]        at (  4/8*\WD@r,0)  (R) {};
        \node[boundarypoint] at ( 10/8*\WD@r,0) (RR) {};
        \draw[doubleline] (LL) -- (L);
        \draw[doubleline] (R) -- (RR);
        \draw[line] (L) to[out= 60, in= 120] (R);
        \draw[line] (L) to[out=-60, in=-120] (R);
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}
%% twice iterated bubble between two free sigma propagators
\NewDocumentCommand{\SigmaFreeBubbleTwice}{s O{1.0}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \node[boundarypoint] at (-10/8*\WD@r,0) (LL) {};
        \node[vertex]        at ( -4/8*\WD@r,0) (L1) {};
        \node[vertex]        at (  4/8*\WD@r,0) (R1) {};
        \node[vertex]        at ( 10/8*\WD@r,0) (L2) {};
        \node[vertex]        at ( 18/8*\WD@r,0) (R2) {};
        \node[boundarypoint] at ( 24/8*\WD@r,0) (RR) {};
        \draw[doubleline] (LL) -- (L1);
        \draw[doubleline] (R1) -- (L2);
        \draw[doubleline] (R2) -- (RR);
        \draw[line] (L1) to[out= 60, in= 120] (R1);
        \draw[line] (L1) to[out=-60, in=-120] (R1);
        \draw[line] (L2) to[out= 60, in= 120] (R2);
        \draw[line] (L2) to[out=-60, in=-120] (R2);
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}
%% bubble diagram
\NewDocumentCommand{\bubbleDiagram}{s O{1.4}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \node[boundarypoint, label={ left:$x\,$}] at (-4/8*\WD@r,0)  (L) {};
        \node[boundarypoint, label={right:$\,y$}] at ( 4/8*\WD@r,0)  (R) {};
        \draw[line] (L) to[out= 60, in= 120] (R);
        \draw[line] (L) to[out=-60, in=-120] (R);
        % \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}

%% sigma propagator
\NewDocumentCommand{\SigmaPropag}{s O{1.2}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \coordinate (L) at (-3/8*\WD@r,0);
        \coordinate (R) at ( 3/8*\WD@r,0);
        \draw[doublefilled] ([yshift=-\WD@dlWidth]L) rectangle ([yshift=+\WD@dlWidth]R);
        \node[boundarypoint] at (L) (e1) {};
        \node[boundarypoint] at (R) (e2) {};
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}
\NewDocumentCommand{\vertexSigma}{s O{1}}{%
    \WD@SetupScaling{\BooleanFalse}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \coordinate (L) at (-3/8*\WD@r,0);
        \coordinate (R) at ( 1/5*\WD@r,0);
        \begin{scope}[overlay, \IfBooleanF{#1}{hide labels}]
            \node[scale=0.1, inner sep=0, label={ 160:$\scriptstyle i$}] at (145:0.9*\WD@r) (e1) {};
            \node[scale=0.1, inner sep=0, label={left:$\scriptstyle j$}] at (215:0.9*\WD@r) (e2) {};
        \end{scope}
        \draw[line] (e1) -- (L);
        \draw[line] (e2) -- (L);
        \IfBooleanTF{#1} %% use either full or free sigma propagator
        {\draw[doubleline] (L) -- (R);}
        {\draw[doublefilled] ([yshift=-\WD@dlWidth]L) rectangle ([yshift=+\WD@dlWidth]R);}
        \node[vertex] at (L) (vL) {};
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}
%% s-exchange Feynman diagram
\NewDocumentCommand{\sExchFeyn}{s O{1}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        % \draw[line] (0,0) circle [radius=\WD@r];
        \coordinate (L) at (-3/8*\WD@r,0);
        \coordinate (R) at ( 3/8*\WD@r,0);
        \WD@BoundaryPoints{#1}
        \draw[line] (e2) -- (L);
        \draw[line] (e1) -- (L);
        \draw[line] (e3) -- (R);
        \draw[line] (e4) -- (R);
        \draw[doublefilled] ([yshift=-\WD@dlWidth]L) rectangle ([yshift=+\WD@dlWidth]R);
        \node[vertex] at (L) (vL) {};
        \node[vertex] at (R) (vR) {};
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}

%% Feynman diagram of bubble chain
\NewDocumentCommand{\bubbleChain}{s O{1}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \coordinate (LL) at (-14/8*\WD@r,0);
        \coordinate  (L) at ( -6/8*\WD@r,0);
        \coordinate  (R) at (  6/8*\WD@r,0);
        \coordinate (RR) at ( 14/8*\WD@r,0);
        \begin{scope}[overlay, \IfBooleanF{#1}{hide labels}]
            \node[boundarypoint] at ([xshift=-11/8*\WD@r]145:\WD@r) (e1) {};
            \node[boundarypoint] at ([xshift=-11/8*\WD@r]215:\WD@r) (e2) {};
            \node[boundarypoint] at ([xshift= 11/8*\WD@r] 35:\WD@r) (e3) {};
            \node[boundarypoint] at ([xshift= 11/8*\WD@r]325:\WD@r) (e4) {};
            \node[anchor=mid, gray] at (0,-0.01) {$\underbrace{\xmathstrut[0.05]{0}\mspace{41mu}{\color{black}\cdots}\mspace{41mu}}_{n \text{ bubbles}}$};
        \end{scope}
        \draw[line, rounded corners=3pt] (e1) -- (LL) -- (e2);
        \draw[line, rounded corners=3pt] (e3) -- (RR) -- (e4);
        \draw[line] ([xshift= 1.2]LL) .. controls +(90:0.25) and +(90:0.25) .. ([xshift=-1.2]L) .. controls +(-90:0.25) and +(-90:0.25) .. ([xshift= 1.2]LL);
        \draw[line] ([xshift=-1.2]RR) .. controls +(90:0.25) and +(90:0.25) .. ([xshift= 1.2]R) .. controls +(-90:0.25) and +(-90:0.25) .. ([xshift=-1.2]RR);
        \draw[line] ([xshift= 1.2]L)++(-60:0.22*\WD@r) .. controls +(140:0.06) and +(-90:0.05) .. ([xshift= 1.2]L) .. controls +( 90:0.06) and +(-140:0.05) .. ++( 60:0.22*\WD@r);
        \draw[dots=2pt, dash phase=0.5pt, lightgray] (L)++(  50:0.25*\WD@r) -- ++(  25:0.22*\WD@r);
        \draw[dots=2pt, dash phase=0.5pt, lightgray] (L)++( -50:0.25*\WD@r) -- ++( -25:0.22*\WD@r);
        \draw[line] ([xshift=-1.2]R)++(120:0.22*\WD@r) .. controls +(-40:0.06) and +( 90:0.05) .. ([xshift=-1.2]R) .. controls +(-90:0.06) and +( 40:0.05) .. ++(-120:0.22*\WD@r);
        \draw[dots=2pt, dash phase=0.5pt, lightgray] (R)++( 130:0.25*\WD@r) -- ++( 155:0.22*\WD@r);
        \draw[dots=2pt, dash phase=0.5pt, lightgray] (R)++(-130:0.25*\WD@r) -- ++(-155:0.22*\WD@r);
        \node[vertexsubtle] at ([xshift= 0.08]LL) (LLV) {};
        \node[vertexsubtle] at ([xshift=-0.05] L)  (LV) {};
        \node[vertexsubtle] at ([xshift= 0.05] R)  (RV) {};
        \node[vertexsubtle] at ([xshift=-0.08]RR) (RRV) {};
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}
%% Exchange Contributions (starred version shows boundary labels)
\NewDocumentCommand{\sExch}{s O{1}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \draw[line] (0,0) circle [radius=\WD@r];
        \coordinate (L) at (-3/8*\WD@r,0);
        \coordinate (R) at ( 3/8*\WD@r,0);
        \WD@BoundaryPoints{#1}
        \draw[line] (e2) -- (L);
        \draw[line] (e1) -- (L);
        \draw[line] (e3) -- (R);
        \draw[line] (e4) -- (R);
        \draw[doublefilled] ([yshift=-\WD@dlWidth]L) rectangle ([yshift=+\WD@dlWidth]R);
        \node[vertex] at (L) (vL) {};
        \node[vertex] at (R) (vR) {};
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}
\NewDocumentCommand{\tExch}{s O{} O{1}}{%
    \WD@SetupScaling{#1}{#3}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \draw[line] (0,0) circle [radius=\WD@r];
        \coordinate (B) at (0,-3/8*\WD@r);
        \coordinate (T) at (0, 3/8*\WD@r);
        \WD@BoundaryPoints{#1}
        \draw[line] (e2) -- (B);
        \draw[line] (e1) -- (T);
        \draw[line] (e3) -- (T);
        \draw[line] (e4) -- (B);
        \draw[doublefilled] ([xshift=-\WD@dlWidth]B) rectangle ([xshift=+\WD@dlWidth]T);
        \node[vertex] at (B) (vB) {};
        \node[vertex] at (T) (vT) {};
        \IfBlankF{#2}{
            \begin{scope}[overlay, inner sep=0, label distance=0.15ex] %% ignore in bounding box calculation
                \node[label={[anchor=mid]200:\(\scriptstyle{#2}\)}] at (0,0) (l) {};
            \end{scope}
        }
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}
\NewDocumentCommand{\uExch}{s O{1}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \draw[line] (0,0) circle [radius=\WD@r];
        \coordinate (B) at (0,-3/8*\WD@r);
        \coordinate (T) at (0, 3/8*\WD@r);
        \WD@BoundaryPoints{#1}
        \draw[line]     (e2) -- (B);
        \draw[line]     (e1) -- (T);
        \draw[line]     (e3) -- (B);
        \draw[overline] (e4) -- (T);
        \draw[doublefilled] ([xshift=-\WD@dlWidth]B) rectangle ([xshift=+\WD@dlWidth]T);
        \node[vertex] at (B) (vB) {};
        \node[vertex] at (T) (vT) {};
        \WD@ExpandBoundingBox % slightly enlarge bounding box
    }
}
\NewDocumentCommand{\sExchHarmonic}{s O{1} O{\D}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \draw[line] (0,0) circle [radius=\WD@r];
        \coordinate (L) at (-4/9*\WD@r,0);
        \coordinate (R) at ( 4/9*\WD@r,0);
        \WD@BoundaryPoints{#1}
        \draw[line] (e2) -- (L);
        \draw[line] (e1) -- (L);
        \draw[line] (e3) -- (R);
        \draw[line] (e4) -- (R);
        \draw[wave=1.5pt] (L) -- (R) node [above,midway]{\(\scriptstyle #3\)};
        \node[bulkpoint] at (L) (vL) {};
        \node[bulkpoint] at (R) (vR) {};
        \WD@ExpandBoundingBox[\WD@xpad][0] % slightly enlarge bounding box
        % \pgfresetboundingbox % if we want to shrink the bounding box, we need to reset it first
        % \useasboundingbox (-\WD@r-\WD@xpad,-\WD@r+1*\WD@ypad) rectangle (\WD@r+\WD@xpad,\WD@r-1*\WD@ypad);
        % \draw (current bounding box.north east) -- (current bounding box.north west) -- (current bounding box.south west) -- (current bounding box.south east) -- cycle;
    }
}
\NewDocumentCommand{\sExchSplit}{s O{1} O{\D} O{\D*}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        \draw[line] (0,0) circle [radius=\WD@r];
        \coordinate (L) at (-4/9*\WD@r,0);
        \coordinate (R) at ( 4/9*\WD@r,0);
        \coordinate (S) at (0,\WD@r);
        \WD@BoundaryPoints{#1}
        \draw[line] (e2) -- (L);
        \draw[line] (e1) -- (L);
        \draw[line] (e3) -- (R);
        \draw[line] (e4) -- (R);
        \draw[line] (L) -- (S) node [above left,  inner sep=-1.7pt, pos=0.5]{\contour*{white}{\(\scriptstyle\scalemath{0.8}{#3}\)}};
        \draw[line] (R) -- (S) node [above right, inner sep=-1.7pt, pos=0.5]{\contour*{white}{\(\scriptstyle\scalemath{0.8}{#4}\)}};
        \node[bulkpoint] at (L) (vL) {};
        \node[bulkpoint] at (R) (vR) {};
        \node[bulkpoint,overlay] at (S) (vS) {};
        \WD@ExpandBoundingBox[\WD@xpad][0] % slightly enlarge bounding box
        % \pgfresetboundingbox % if we want to shrink the bounding box, we need to reset it first
        % \useasboundingbox (-\WD@r-\WD@xpad,-\WD@r+1*\WD@ypad) rectangle (\WD@r+\WD@xpad,\WD@r-1*\WD@ypad);
        % \draw (current bounding box.north east) -- (current bounding box.north west) -- (current bounding box.south west) -- (current bounding box.south east) -- cycle;
    }
}

%%% Partial Waves

%% Padding around Partial Waves
\NewExpandableDocumentCommand{\PW@rDefault}{}{\WD@rDefault}
\NewExpandableDocumentCommand{\PW@xpadDefault}{}{0.15em}
%% Helper macro to set the scaling factor for Partial Waves
\NewDocumentCommand{\PW@SetupScaling}{m}{% #1: scaling factor
    \def\WD@r{#1*\PW@rDefault}
    \def\PW@xpad{#1*\PW@xpadDefault}
}

\NewDocumentCommand{\shadowRepCPW}{s O{1} O{\D} O{\D*}}{%
    \WD@SetupScaling{#1}{#2}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}]{
        % \draw[line] (0,0) circle [radius=\WD@r];
        \coordinate (L) at (-7/8*\WD@r,0);
        \coordinate (R) at ( 7/8*\WD@r,0);
        \coordinate (S) at (0,0);
        \begin{scope}[overlay, \IfBooleanF{#1}{hide labels}]
            \node[boundarypoint] at ([xshift=-4/8*\WD@r]145:\WD@r) (e1) {};
            \node[boundarypoint] at ([xshift=-4/8*\WD@r]215:\WD@r) (e2) {};
            \node[boundarypoint] at ([xshift= 4/8*\WD@r] 35:\WD@r) (e3) {};
            \node[boundarypoint] at ([xshift= 4/8*\WD@r]325:\WD@r) (e4) {};
        \end{scope}
        \draw[thinline] (e2) -- (L);
        \draw[thinline] (e1) -- (L);
        \draw[thinline] (e3) -- (R);
        \draw[thinline] (e4) -- (R);
        \draw[thinline] (L) -- (S) node [xshift= 1/13*\WD@r, above, inner sep=1pt, midway]{\(\scriptstyle #3\)};
        \draw[thinline] (R) -- (S) node [xshift=-1/13*\WD@r, above, inner sep=1pt, midway]{\(\scriptstyle #4\)};
        \node[opevertex,scale=2] at (L) (vL) {};
        \node[opevertex,scale=2] at (R) (vR) {};
        \node[bulkpoint] at (S) (vS) {};
        \WD@ExpandBoundingBox[3*\WD@xpad] % slightly enlarge bounding box
    }
}

%% BUG: need to explicitely set black color, otherwise \mathcolor command
%%      can change it in a weird way (even when this macro is used outside)
\NewDocumentCommand{\sPartWave}{s O{\D} O{J} O{1}}{%
    \PW@SetupScaling{#4}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}, color=black]{
        \node[opevertex] at (-1/2*\WD@r,0) (vL) {};
        \node[opevertex] at ( 1/2*\WD@r,0) (vR) {};
        \draw[thinline] (215:\WD@r) -- (vL);
        \draw[thinline] (145:\WD@r) -- (vL);
        \draw[thinline] ( 35:\WD@r) -- (vR);
        \draw[thinline] (325:\WD@r) -- (vR);
        \draw[thickline] (vL) -- (vR);
        \begin{scope}[overlay, inner sep=0, label distance=0.1ex] %% ignore in bounding box calculation
            \node[label={[above]\(\scriptstyle\IfBooleanF{#1}{#2\IfBlankF{#3}{,\.#3}}\)}] at (0,0) (l) {};
        \end{scope}
        \WD@ExpandBoundingBox[\PW@xpad][0] % slightly enlarge bounding box
    }
}
\NewDocumentCommand{\tPartWave}{s O{\Dpr} O{J'} O{1}}{%
    \PW@SetupScaling{#4}
    \tikz[baseline={([yshift=-0.6ex]current bounding box.center)}, color=black]{
        \node[opevertex] at (0,-1/3*\WD@r) (vB) {};
        \node[opevertex] at (0, 1/3*\WD@r) (vT) {};
        \draw[thinline] (215:\WD@r) -- (vB);
        \draw[thinline] (145:\WD@r) -- (vT);
        \draw[thinline] ( 35:\WD@r) -- (vT);
        \draw[thinline] (325:\WD@r) -- (vB);
        \draw[thickline] (vB) -- (vT);
        \begin{scope}[overlay, inner sep=0, label distance=0.15ex] %% ignore in bounding box calculation
            \node[label={[anchor=mid west]right:\(\scriptstyle\IfBooleanF{#1}{#2\IfBlankF{#3}{\mspace{-2mu},\.#3}}\)}] at (0,0) (l) {};
        \end{scope}
        \WD@ExpandBoundingBox[\PW@xpad][0] % slightly enlarge bounding box
    }
}

